Towards an Atlas of Cultural Commonsense for Machine Reasoning

Existing commonsense reasoning datasets for AI and NLP tasks fail to address an important aspect of human life: cultural differences. We introduce an approach that extends prior work on crowdsourcing commonsense knowledge by incorporating differences in knowledge that are attributable to cultural or national groups. We demonstrate the technique by collecting commonsense knowledge that surrounds six fairly universal rituals -- birth, coming-of-age, marriage, funerals, new year, and birthdays -- across two national groups: the United States and India. Our study expands the different types of relationships identified by existing work in the field of commonsense reasoning for commonplace events, and uses these new types to gather information that distinguish the identity of the groups providing the knowledge. It also moves us a step closer towards building a machine that doesn't assume a rigid framework of universal (and likely Western-biased) commonsense knowledge, but rather has the ability to reason in a contextually and culturally sensitive way. Our hope is that cultural knowledge of this sort will lead to more human-like performance in NLP tasks such as question answering (QA) and text understanding and generation.

==> pgf-pie/before-after-number.tex <==
\begin{tikzpicture}
  \pie[before number={\$}, after number=,]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/cloud.tex <==
\begin{tikzpicture}
  \pie[cloud, text=inside, scale font]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/color.tex <==
\begin{tikzpicture}
  \pie[color={black!10, black!20, black!30, black!40}]
  {10/A, 20/B, 30/C, 40/D}

  \pie[pos={8,0}, color=blue!20] {10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}


==> pgf-pie/colorwheel.tex <==
\begin{tikzpicture}
  \pie{10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/}
\end{tikzpicture}

==> pgf-pie/explode.tex <==
\begin{tikzpicture}
  % explode list
  \pie[explode={0, 0, 0, 0.1}] {10/A, 20/B, 30/C, 40/D}

  % explode all
  \pie[pos={8,0}, explode=0.1] {10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/first-pie.tex <==
\begin{tikzpicture}
  \pie{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/hide-number.tex <==
\begin{tikzpicture}
  \pie[hide number]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}


==> pgf-pie/legend.tex <==
\begin{tikzpicture}
  \pie[text=legend]{10/First, 20/Second, 30/Third, 40/Fourth}
\end{tikzpicture}

==> pgf-pie/polar.tex <==
\begin{tikzpicture}
  \pie[polar]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/population.tex <==
% data from http://en.wikipedia.org/wiki/List_of_countries_by_population
\begin{tikzpicture}
  \pie[cloud, rotate=45, sum=auto, radius=35, after number=, text=pin] {1339/China,
    1210/India, 312/USA, 237/Indonesia, 190/Brazil, 177/Pakistan,
    158/Nigeria, 151/Bangladesh, 142/Russia, 127/Japan, 112/Mexico,
    94/Philippines, 87/Vietnam, 82/Ethiopia, 81/Germany, 80/Egypt,
    75/Iran, 73/Turkey, 67/Thailand, 65/Congo, 65/France, 62/UK,
    60/Italy, 50/South Africa, 48/South Korea, 47/Myanmar, 46/Spain,
    46/Colombia, 45/Ukraine, 43/Tanzania, 40/Argentina, 38/Kenya,
    38/Poland, 36/Algeria, 34/Canada, 32/Morocco, 31/Uganda, 31/Iraq,
    31/Afghanistan, 30/Sudan, 29/Peru, 29/Venezuela, 28/Nepal,
    28/Malaysia, 27/Uzbekistan, 27/Saudi Arabia, 24/Ghana, 24/North
    Korea, 23/Syria, 23/Taiwan, 22/Australia, 22/Yemen, 21/Romania,
    20/Madagascar, 20/Sri Lanka, 20/Mozambique, 19/Cote d'Ivoire,
    19/Cameroon, 19/Angola, 17/Chile, 16/Netherlands, 16/Kazakhstan,
    15/Burkina Faso, 15/Niger, 14/Malawi, 14/Mali, 14/Guatemala,
    14/Ecuador, 13/Cambodia, 13/Zambia, 12/Zimbabwe, 12/Senegal,
    11/Cuba, 11/Chad, 10/Belgium, 10/Greece, 10/Portugal, 10/Tunisia,
    10/Czech Republic, 10/Bolivia, 10/Rwanda, 10/Haiti, 10/Hungary,
    10/Guinea, 10/Belarus, 9/Sweden, 9/Dominican Republic, 9/Somalia,
    9/Azerbaijan, 9/Benin, 8/Austria, 8/Burundi, 8/United Arab
    Emirates, 8/South Sudan, 8/Honduras, 8/Switzerland, 8/Israel,
    7/Bulgaria, 7/Serbia, 7/Hong Kong }

  % \node[circle,draw=black,thick, fill=white, font=\bf]
  % {Population of the world};
\end{tikzpicture}


==> pgf-pie/radius.tex <==
\begin{tikzpicture}
  \pie{10/, 20/, 30/, 40/}

  \pie[pos={8,0}, rotate=180]{10/, 20/, 30/, 40/}

  \pie[pos={17,0}, radius=4]{10/, 20/, 30/, 40/}
\end{tikzpicture}

==> pgf-pie/scalefont.tex <==
\begin{tikzpicture}
  \pie[scale font]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/shadow.tex <==
% \usetikzlibrary{shadows}
\begin{tikzpicture}
  \pie[style=drop shadow]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}


==> pgf-pie/square.tex <==
\begin{tikzpicture}
  \pie[square]{40/A, 30/B, 20/C, 10/D}
\end{tikzpicture}

==> pgf-pie/sum.tex <==
\begin{tikzpicture}
  \pie[sum=auto, after number=, radius=2]{33/Boys, 7/Girls}

  \pie[pos={6,0}, sum=40, after number=, radius=2]{33/Boys}
\end{tikzpicture}

==> pgf-pie/text-inside.tex <==
\begin{tikzpicture}
  \pie[text=inside]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> pgf-pie/text.tex <==
\begin{tikzpicture}
  \pie[text=pin]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> title-brainstorming.tex <==
culture
ritual
logic
embedded
atlas
machine reasoning
commonsense
if-then reasoning
customs



ATOMIC - Atlas of Machine Commonsense for If-Then Reasoning
NUCLEAR
MOLECULAR
ELECTRON
PROTON
NEUTRON
ISOTOPE / ISOTOPIC
high-atomic weight : Heavy elements

ATOMIC : us :: atom :: ?
+adding culture

An Atlas of Ritual Commonsense for Machine Reasoning 

ASTEROID
Atlas
of 
Ritual


New
Updated
Cultural
Logic
Embedded
Atlas (of/for)
Rituals/Reasoning

